Uniform asymptotic estimates of transition probabilities on combs

We investigate the asymptotical behaviour of the transition probabilities of the simple random walk on the 2-comb. In particular we obtain space-time uniform asymptotical estimates which show the lack of symmetry of this walk better than local limit estimates. Our results also point out the impossibility of getting Jones-type non-Gaussian estimates.

==> coman.tex <==
%file macrodario.tex


\catcode`@=11
%
%------------------------- comandi riservati ---------------------------
%
\def\b@lank{ }

\newif\if@simboli
\newif\if@riferimenti
\newif\if@bozze
\newif\if@data



\def\bozze{\@bozzetrue
\immediate\write16{!!!   INSERISCE NOME EQUAZIONI   !!!}}


\newwrite\file@simboli
\def\simboli{

    \immediate\write16{ !!! Genera il file \jobname.SMB }
    \@simbolitrue\immediate\openout\file@simboli=\jobname.smb
     \immediate\write\file@simboli{Simboli di \jobname}}

\newwrite\file@ausiliario
\def\riferimentifuturi{
    \immediate\write16{ !!! Genera il file \jobname.aux }
    \@riferimentitrue\openin1 \jobname.aux
    \ifeof1\relax\else\closein1\relax\input\jobname.aux\fi
    \immediate\openout\file@ausiliario=\jobname.aux}

\newcount\eq@num\global\eq@num=0
\newcount\sect@num\global\sect@num=0
\newcount\para@num\global\para@num=0
\newcount\lemm@num\global\lemm@num=0


\newif\if@ndoppia
\def\numerazionedoppia{\@ndoppiatrue\gdef\la@sezionecorrente{\the\sect@num}}

\def\se@indefinito#1{\expandafter\ifx\csname#1\endcsname\relax}
\def\spo@glia#1>{} % si applica a \meaning\xxxxx; butta via tutto quello
                   % che produce \meaning fino al carattere >
                   % (v. manuale TeX, pag. 382, \strip#1>{}).

\newif\if@primasezione
\@primasezionetrue

\def\s@ection#1\par{\immediate
    \write16{#1}\if@primasezione\global\@primasezionefalse\else\goodbreak
    \vskip\spaziosoprasez\fi\noindent
    {\bf#1}\nobreak\vskip\spaziosottosez\nobreak\noindent}

%--------------------------- Indice -------------------------------


\newif\if@indice
\newif\if@ceindice

\newwrite\file@indice

\def\indice{
           \immediate\write16{Genera il file \jobname.ind}
           \@indicetrue
           \immediate\openin2 \jobname.ind
           \ifeof2\relax\else
             \closein2\relax
       \@ceindicetrue\fi
            \if@ceindice\relax\else
            \immediate\openout\file@indice=\jobname.ind
         \immediate\write
         \file@indice{\string\vskip5pt
         \string{ \string\bf \string\centerline\string{ Indice
         \string}\string}\string\par}
            \fi
            }

\def\quiindice{\if@ceindice\vfill\eject\input\jobname.ind\else\vfill\eject
       \immediate\write\file@indice{\string{\string\bf\string~
       Indice\string}\string\hfill\folio}
       \null\vfill\eject\null\vfill\eject\relax\fi}

%

%------------------------------ a disp. dell'utente:  sezioni -------------

\def\sezpreset#1{\global\sect@num=#1
    \immediate\write16{ !!! sez-preset = #1 }   }

\def\spaziosoprasez{50pt plus 60pt}
\def\spaziosottosez{15pt}

\def\sref#1{\se@indefinito{@s@#1}\immediate\write16{ ??? \string\sref{#1}
    non definita !!!}
    \expandafter\xdef\csname @s@#1\endcsname{??}\fi\csname @s@#1\endcsname}

\def\autosez#1#2\par{
    \global\advance\sect@num by 1\if@ndoppia\global\eq@num=0\fi
    \global\lemm@num=0
    \global\para@num=0
    \xdef\la@sezionecorrente{\the\sect@num}
    \def\usa@getta{1}\se@indefinito{@s@#1}\def\usa@getta{2}\fi
    \expandafter\ifx\csname @s@#1\endcsname\la@sezionecorrente\def
    \usa@getta{2}\fi
    \ifodd\usa@getta\immediate\write16
      { ??? possibili riferimenti errati a \string\sref{#1} !!!}\fi
    \expandafter\xdef\csname @s@#1\endcsname{\la@sezionecorrente}
    \immediate\write16{\la@sezionecorrente. #2}
    \if@simboli
      \immediate\write\file@simboli{ }\immediate\write\file@simboli{ }
      \immediate\write\file@simboli{  Sezione
                                  \la@sezionecorrente :   sref.   #1}
      \immediate\write\file@simboli{ } \fi
    \if@riferimenti
      \immediate\write\file@ausiliario{\string\expandafter\string\edef
      \string\csname\b@lank @s@#1\string\endcsname{\la@sezionecorrente}}\fi
    \goodbreak\vskip 20pt plus 20pt
    \noindent{\bf\the\sect@num.\quad #2}
   \if@bozze
    {\tt #1}\fi
    \par\nobreak\vskip 15pt
    \nobreak}

\def\blankii{\blank\blank}

\def\destra#1{{\hfill#1}}
\font\titfnt=cmbx12 scaled \magstep2
\font\capfnt=cmbx12 scaled \magstep2
\def\blank{\vskip 12pt}

\def\capitolo#1#2\par{
    \global\advance\sect@num by 1\if@ndoppia\global\eq@num=0\fi
    \global\lemm@num=0
    \global\para@num=0
    \xdef\la@sezionecorrente{\the\sect@num}
    \def\usa@getta{1}\se@indefinito{@s@#1}\def\usa@getta{2}\fi
    \expandafter\ifx\csname @s@#1\endcsname\la@sezionecorrente\def
    \usa@getta{2}\fi
    \ifodd\usa@getta\immediate\write16
      { ??? possibili riferimenti errati a \string\sref{#1} !!!}\fi
    \expandafter\xdef\csname @s@#1\endcsname{\la@sezionecorrente}
    \immediate\write16{\la@sezionecorrente. #2}
   \if@simboli
      \immediate\write\file@simboli{ }\immediate\write\file@simboli{ }
      \immediate\write\file@simboli{  Sezione
                                  \la@sezionecorrente :   sref.   #1}
      \immediate\write\file@simboli{ } \fi
    \if@riferimenti
      \immediate\write\file@ausiliario{\string\expandafter\string\edef
      \string\csname\b@lank @s@#1\string\endcsname{\la@sezionecorrente}}\fi
           \par\vfill\eject
           \destra{\capfnt {}\hbox to 10pt{\hfil}}
           \blankii\noindent{\titfnt\baselineskip=20pt
           \hfill{#2}}\blankii
      \if@indice
       \if@ceindice\relax\else\immediate\write
       \file@indice{\string\vskip5pt\string{\string\bf
       \la@sezionecorrente.#2\string}\string\hfill\folio\string\par}\fi\fi
       \if@bozze
         {\tt #1}\par\fi\nobreak}

                    


\def\semiautosez#1#2\par{
    \gdef\la@sezionecorrente{#1}\if@ndoppia\global\eq@num=0\fi
    \if@simboli
      \immediate\write\file@simboli{ }\immediate\write\file@simboli{ }
      \immediate\write\file@simboli{  Sezione ** : sref.
          \expandafter\spo@glia\meaning\la@sezionecorrente}
      \immediate\write\file@simboli{ }\fi
    \s@ection#2\par}


%------------------paragrafi----------------------------------------


\def\pararef#1{\se@indefinito{@ap@#1}
    \immediate\write16{??? \string\pararef{#1} non definito !!!}
    \expandafter\xdef\csname @ap@#1\endcsname {#1}
    \fi\csname @ap@#1\endcsname}

\def\autopara#1#2\par{
     \global\advance\para@num by 1
     \xdef\il@paragrafo{\la@sezionecorrente.\the\para@num}
     \vskip10pt
     \noindent {\bf \il@paragrafo\ #2}
     \def\usa@getta{1}\se@indefinito{@ap@#1}\def\usa@getta{2}\fi
     \expandafter\ifx\csname
@ap@#1\endcsname\il@paragrafo\def\usa@getta{2}\fi
     \ifodd\usa@getta\immediate\write16
        {??? possibili riferimenti errati a \string\pararef{#1} !!!}\fi
     \expandafter\xdef\csname @ap@#1\endcsname{\il@paragrafo}
     \def\usa@getta{\expandafter\spo@glia\meaning
     \la@sezionecorrente.\the\para@num}
     \if@simboli
      \immediate\write\file@simboli{ }\immediate\write\file@simboli{ }
      \immediate\write\file@simboli{ paragrafo
                                  \il@paragrafo :   pararef.   #1}
      \immediate\write\file@simboli{ } \fi
    \if@riferimenti
      \immediate\write\file@ausiliario{\string\expandafter\string\edef
      \string\csname\b@lank @ap@#1\string\endcsname{\il@paragrafo}}\fi
    \if@indice
     \if@ceindice\relax\else\immediate\write
       \file@indice{\string\noindent\string\item\string{
       \il@paragrafo.\string}#2\string\dotfill\folio\string\par}\fi\fi
    \if@bozze
       {\tt #1}\fi\par\nobreak\vskip .3 cm \nobreak}

%------------------------------ a disp. dell'utente:  equazioni -----------


\def\eqpreset#1{\global\eq@num=#1
     \immediate\write16{ !!! eq-preset = #1 }     }

\def\eqlabel#1{\global\advance\eq@num by 1
    \if@ndoppia\xdef\il@numero{\la@sezionecorrente.\the\eq@num}
       \else\xdef\il@numero{\the\eq@num}\fi
    \def\usa@getta{1}\se@indefinito{@eq@#1}\def\usa@getta{2}\fi
    \expandafter\ifx\csname @eq@#1\endcsname\il@numero\def\usa@getta{2}\fi
    \ifodd\usa@getta\immediate\write16
       { ??? possibili riferimenti errati a \string\eqref{#1} !!!}\fi
    \expandafter\xdef\csname @eq@#1\endcsname{\il@numero}
    \if@ndoppia
       \def\usa@getta{\expandafter\spo@glia\meaning
       \il@numero}
       \else\def\usa@getta{\il@numero}\fi
    \if@simboli
       \immediate\write\file@simboli{  Equazione
            \usa@getta :  eqref.   #1}\fi
    \if@riferimenti
       \immediate\write\file@ausiliario{\string\expandafter\string\edef
       \string\csname\b@lank @eq@#1\string\endcsname{\usa@getta}}\fi}

\def\eqsref#1{\se@indefinito{@eq@#1}
    \immediate\write16{ ??? \string\eqref{#1} non definita !!!}
    \if@riferimenti\relax
    \else\eqlabel{#1} ???\fi
    \fi\csname @eq@#1\endcsname }

\def\autoeqno#1{\eqlabel{#1}\eqno(\csname @eq@#1\endcsname)\if@bozze
        {\tt #1}\else\relax\fi}
\def\autoleqno#1{\eqlabel{#1}\leqno(\csname @eq@#1\endcsname)}
\def\eqref#1{(\eqsref{#1})}

%----------- Lemmi automatici: a disposizione dell'utente ----------------

\def\lemmalabel#1{\global\advance\lemm@num by 1
    \xdef\il@lemma{\la@sezionecorrente.\the\lemm@num}
    \def\usa@getta{1}\se@indefinito{@lm@#1}\def\usa@getta{2}\fi
    \expandafter\ifx\csname @lm@#1\endcsname\il@lemma\def\usa@getta{2}\fi
    \ifodd\usa@getta\immediate\write16
       { ??? possibili riferimenti errati a \string\lemmaref{#1} !!!}\fi
    \expandafter\xdef\csname @lm@#1\endcsname{\il@lemma}
    \def\usa@getta{\expandafter\spo@glia\meaning
       \la@sezionecorrente.\the\lemm@num}
       \if@simboli
       \immediate\write\file@simboli{  Lemma
            \usa@getta :  lemmaref #1}\fi
    \if@riferimenti
       \immediate\write\file@ausiliario{\string\expandafter\string\edef
       \string\csname\b@lank @lm@#1\string\endcsname{\usa@getta}}\fi}

\def\autolemma#1{\lemmalabel{#1}\csname @lm@#1\endcsname\if@bozze
    {\tt #1}\else\relax\fi}

\def\lemmaref#1{\se@indefinito{@lm@#1}
    \immediate\write16{ ??? \string\lemmaref{#1} non definita !!!}
    \if@riferimenti\else
    \lemmalabel{#1}???\fi
    \fi\csname @lm@#1\endcsname}


%--------------- bibliografia automatica: riservati ----------------------


\newcount\cit@num\global\cit@num=0

\newwrite\file@bibliografia
\newif\if@bibliografia
\@bibliografiafalse
\newif\if@corsivo
\@corsivofalse

\def\title#1{\centerline{\bf #1}}
\def\rivista#1{#1}

\def\lp@cite{[}
\def\rp@cite{]}
\def\trap@cite#1{\lp@cite #1\rp@cite}
\def\lp@bibl{[}
\def\rp@bibl{]}
\def\trap@bibl#1{\lp@bibl #1\rp@bibl}

\def\refe@renza#1{\if@bibliografia\immediate        % scrive su .BIB
    \write\file@bibliografia{
    \string\item{\trap@bibl{\cref{#1}}}\string
    \bibl@ref{#1}\string\bibl@skip}\fi}

\def\ref@ridefinita#1{\if@bibliografia\immediate\write\file@bibliografia{
    \string\item{?? \trap@bibl{\cref{#1}}} ??? tentativo di ridefinire la
      citazione #1 !!! \string\bibl@skip}\fi}

\def\bibl@ref#1{\se@indefinito{@ref@#1}\immediate
    \write16{ ??? biblitem #1 indefinito !!!}\expandafter\xdef
    \csname @ref@#1\endcsname{ ??}\fi\csname @ref@#1\endcsname}

\def\c@label#1{\global\advance\cit@num by 1\xdef            % assegna il numero
   \la@citazione{\the\cit@num}\expandafter
   \xdef\csname @c@#1\endcsname{\la@citazione}}

\def\bibl@skip{\vskip 5truept}

%------------------------ bibl. automatica: a disp. dell'utente ------------

\def\stileincite#1#2{\global\def\lp@cite{#1}\global
    \def\rp@cite{#2}}
\def\stileinbibl#1#2{\global\def\lp@bibl{#1}\global
    \def\rp@bibl{#2}}

\def\corsivo{\global\@corsivotrue}

\def\citpreset#1{\global\cit@num=#1
    \immediate\write16{ !!! cit-preset = #1 }    }

\def\autobibliografia{\global\@bibliografiatrue\immediate
    \write16{ !!! Genera il file \jobname.BIB}\immediate
    \openout\file@bibliografia=\jobname.bib}

\def\cref#1{\se@indefinito                  % se indefinito definisce
   {@c@#1}\c@label{#1}\refe@renza{#1}\fi\csname @c@#1\endcsname}
\def\upcref#1{\null$^{\,\cref{#1}}$}

\def\cite#1{\trap@cite{\cref{#1}}}                  %  [5]
\def\ccite#1#2{\trap@cite{\cref{#1},\cref{#2}}}     %  [5,6]
\def\ncite#1#2{\trap@cite{\cref{#1}--\cref{#2}}}    %  [5-8] senza definire
\def\upcite#1{$^{\,\trap@cite{\cref{#1}}}$}               % ^[5]
\def\upccite#1#2{$^{\,\trap@cite{\cref{#1},\cref{#2}}}$}  % ^[5,6]
\def\upncite#1#2{$^{\,\trap@cite{\cref{#1}-\cref{#2}}}$}  % ^[5-8] senza def.

\def\clabel#1{\se@indefinito{@c@#1}\c@label           % sola definizione
    {#1}\refe@renza{#1}\else\c@label{#1}\ref@ridefinita{#1}\fi}
\def\cclabel#1#2{\clabel{#1}\clabel{#2}}                     % def. doppia
\def\ccclabel#1#2#3{\clabel{#1}\clabel{#2}\clabel{#3}}       % def. tripla

\def\biblskip#1{\def\bibl@skip{\vskip #1}}           % spaziatura nella bibl.

\def\insertbibliografia{\if@bibliografia             % scrive la bibliografia
    \immediate\write\file@bibliografia{ }
    \immediate\closeout\file@bibliografia
   \if@indice
     \if@ceindice\relax\else\immediate\write
       \file@indice{\string\vskip5pt\string{\string\bf\string~
       Bibliografia\string}\string\hfill\folio\string\par}\fi\fi
     \catcode`@=11\input\jobname.bib\catcode`@=12\fi
   }

%--------- per comporre il file con la bibliografia --------------

\def\commento#1{\relax}
\def\biblitem#1#2\par{\expandafter\xdef\csname @ref@#1\endcsname{#2}}

% ricordare: una lista in chiaro della bibliografia si
% ottiene eseguendo $ TEX BIBLIST



%------------------ FORMATI TEOREMI E GENERALI --------------------

\def\abstract{
\vskip48pt plus 60pt
\noindent
{\bf Abstract.}}

\def\summary{
\centerline{{\bf Summary.}}\par}

\def\firma{\noindent
\centerline{D.~Bertacchi - F.~Zucca}\par\noindent
\centerline{Universit\`a degli Studi di Milano}\par\noindent
\centerline{Dipartimento di Matematica F.~Enriques}\par\noindent
\centerline{Via Saldini 50, 20133 Milano, Italy.}\par}


\def\theorem#1#2{\par\vskip4pt
{\bf Theorem \autolemma{#1}.}{\it \ #2}
 \par\vskip10pt}

\def\teofin{\par\vskip10pt}

\def\lemma#1#2{\par\vskip4pt
{\bf Lemma \autolemma{#1}.}{\it \ #2}
 \par\vskip4pt}


\def\proof{\par\noindent{\sl Proof.}\ }

\def\proposition#1#2{\par\vskip4pt
{\bf Proposition \autolemma{#1}.}{\it \ #2}
 \par\vskip10pt}
\def\corollary#1#2{\par\vskip4pt
{\bf Corollary \autolemma{#1}.}{\it \ #2}
 \par\vskip10pt}

\def\remark#1#2{\par\vskip4pt
{\bf Remark \autolemma{#1}.}{\ #2}
 \par\vskip4pt}

\def\definition#1#2{\par\vskip4pt
{\bf Definition \autolemma{#1}.}{\it \ #2}
 \par\vskip4pt}

\def\assumption#1#2{\par\vskip4pt
{\bf Assumption \autolemma{#1}.}{\it \ #2}
 \par\vskip4pt}

\def\example#1#2{\par\vskip4pt
{\bf Example \autolemma{#1}.}{\ #2}
 \par\vskip4pt}


\def\quadratino{\nobreak\par\nobreak
\hfill\vbox{\hrule\hbox{\vrule\vbox to 7 pt {\vfill\hbox to
7 pt {\hfill\hfill}\vfill}\vrule}\hrule}\par}

%------------------------------ F I N E ---------------------------------

